Centroid Distance Distillation for Effective Rehearsal in Continual Learning

Rehearsal, retraining on a stored small data subset of old tasks, has been proven effective in solving catastrophic forgetting in continual learning. However, due to the sampled data may have a large bias towards the original dataset, retraining them is susceptible to driving continual domain drift of old tasks in feature space, resulting in forgetting. In this paper, we focus on tackling the continual domain drift problem with centroid distance distillation. First, we propose a centroid caching mechanism for sampling data points based on constructed centroids to reduce the sample bias in rehearsal. Then, we present a centroid distance distillation that only stores the centroid distance to reduce the continual domain drift. The experiments on four continual learning datasets show the superiority of the proposed method, and the continual domain drift can be reduced.

==> rel.tex <==
\section{Related Work}


\noindent
\textbf{Continual learning.}
% Continuous learning aims to solve the catastrophic forgetting problem caused by not saving or saving a small amount of old task data. 
Current CL methods can be divided into three categories.
% regularization-based, parameter-isolation and Replay-based methods.
First, regularization-based methods~\cite{5,11,hinton2015distilling} impose constraints on model updates through regularization to alleviate catastrophic forgetting. 
% Earlier methods imposed constraints on model parameters or gradients during optimization by adding a penalty term to the loss function~\cite{5,11}.
Parameter-isolation methods~\cite{16,15,xu2018reinforced} adapt to new tasks by dynamically adding new nodes or new layers to the neural network. 
% By changing the way of network architecture, the mutual influence between weights is reduced and the mutual interference between tasks is reduced~\cite{16}\cite{15}.
Rehearsal-based methods~\cite{8,7,Shim2021,6,17} review knowledge of old tasks by generating or retaining a small amount of old task data.
% Nowadays, replay-based methods pay more and more attention to the problem of memory sample selection.
% iCARL averages the eigenvalues of the training data and selects the data closest to the mean~\cite{8}.
% Ticker selects samples with large entropy in the data stream~\cite{7}.
% ASER selects samples near the decision boundary\cite{Shim2021}.
The existing rehearsal methods always randomly select the sample to be stored, such as reservoir sampling and ring buffer sampling~\cite{6}.
% RM propose a memory management strategy based on per-sample classification uncertainty and data augmentation~\cite{17}.
% ASER stores samples near the classification boundary by calculating the adversarial shapely value~\cite{Shim2021}. 
% Because memory storage is expensive, how to select samples is the core problem of the replay-based method.
Unfortunately, the randomly selected samples may have large biases, and directly retraining on biased memory is susceptible to forgetting due to the continual domain shift.

\noindent
\textbf{Continual domain drift.}
In CL, the distribution of old tasks on feature space gets shifted during the training of new tasks.
The phenomenon is named continual domain shift.
The rehearsal stores a very small number of old task samples relative to the new task datasets.
However, retraining on the biased selected samples results in over-fitting and indistinguishable because of the continual domain shift.
%so the feature of the old task is inevitably transferred to the new task, resulting in the phenomenon of domain overlap. 
The continual domain shift results in catastrophic forgetting. 
In the latest study, MDMT-R augments and constrains the classification boundaries by margin loss and distillation~\cite{3}.
SCR mitigates the effect of continual domain drift by increasing the inter-class distance through a supervised contrastive loss~\cite{2}. 
In this paper, we propose to tackle the forgetting raised by continual domain shift in the perspective of stored data.
We study to select data and make full use of the stored information.
